SCOPE: Secure Compiling of PLCs in Cyber-Physical Systems

Cyber-Physical Systems (CPS) are being widely adopted in critical infrastructures, such as smart grids, nuclear plants, water systems, transportation systems, manufacturing and healthcare services, among others. However, the increasing prevalence of cyberattacks targeting them raises a growing security concern in the domain. In particular, memory-safety attacks, that exploit memory-safety vulnerabilities, constitute a major attack vector against real-time control devices in CPS. Traditional IT countermeasures against such attacks have limitations when applied to the CPS context: they typically incur in high runtime overheads; which conflicts with real-time constraints in CPS and they often abort the program when an attack is detected, thus harming availability of the system, which in turn can potentially result in damage to the physical world. In this work, we propose to enforce a full-stack memory-safety (covering user-space and kernel-space attack surfaces) based on secure compiling of PLCs to detect memory-safety attacks in CPS. Furthermore, to ensure availability, we enforce a resilient mitigation technique that bypasses illegal memory access instructions at runtime by dynamically instrumenting low-level code. We empirically measure the computational overhead caused by our approach on two experimental settings based on real CPS. The experimental results show that our approach effectively and efficiently detects and mitigates memory-safety attacks in realistic CPS.

==> 03_background.tex <==
\section{Background}\label{background}

In this section, we provide background information of some of the relevant topics and technologies used in this research work. In particular, this section presents a background information of cyber-physical systems (CPS), \revise{the CPS testbeds used for experimentation (i.e. SWaT and SecUTS)}. %, memory-safety attacks and the existing memory-safety tools enforced to our CPS testbeds (i.e. ASan and KASan). 

\subsection{Overview of CPS}\label{cps_overview}

%\subsection{History} %% tobod added later

%Cyber-physical systems are the current computing trends that are extended from the traditional embedded systems. 

%They are widely applicable in mission-critical infrastructures such as smart grid systems, water treatment and distribution systems, healthcare systems, nuclear plants, automotive systems, military systems, robotics, industrial automations, manufacturing, smart buildings, and so on. 

%The fundamental challenge in CPS is ...

%\subsection{Architecture}\label{cps_architecture}

%Unlike traditional IT systems, CPS involves complex interactions among various entities while integrating physical plants and control devices (PLCs) via communication networks. 
Unlike traditional IT systems, CPS involves complex interactions between entities in the physical space and the cyber space over communication networks. Such complex interactions are accomplished via communication with the physical world via sensors and actuators and with the digital world via controllers (PLCs) and other embedded devices. These interactions are also constrained by hard deadlines. Missing deadlines could result in disruption of control-loop stability or a complete system failure (in the worst case) since it could cause the underlying system to run into an unstable and unsafe state. This makes CPS highly real-time constrained systems. %\revise{The CPS design constraints (including real-time constraints and physical-state resiliency) are briefly modeled in Chapter \ref{chapter3}}. 
The edge devices in a typical CPS are also highly resource constrained devices. For example, PLCs and input/output devices have restricted storage capacity (e.g. limited RAM size) and computational power (e.g. limited CPU speed).  %Since these devices run for long time without rebooting, the probability of getting buffer overflows is also high, which could result system failures or severe vulnerabilities for cyber attacks. 
%CPS usually impose hard real-time constraints. If such real-time constraints are not met, then the underlying system might run into an unstable and unsafe state. Moreover, 

In general, a typical CPS consists of the following entities:
\begin{itemize}
\item \textit{Physical plants}: physical entities where the physical processes take place.
\item \textit{Sensors}: devices that are capable of reading or observing state information of plants and physical processes which will be later used as inputs for controllers (PLCs).
\item \textit{PLCs}: control devices that that receive sensor inputs, make decisions (based on inputs obtained from sensors) and issue control commands to actuators. These control commands will help to control actual processes of the physical plant when they are implemented by actuators. 
\item \textit{Actuators}: physical entities that are capable of implementing the control commands issued by the PLCs.
\item  \textit{Supervisory control and data acquisition (SCADA)}: a software entity designed for monitoring and controlling different processes in a CPS. It often comprises a human-machine interface (HMI) and a historian server. The HMI is used to display state information of plants and physical processes in the CPS.  The historian server is used to store all operational data, alarm history and events.    
\item  \textit{Communication networks}: communication medias where packets (containing sensor measurements, control commands, alarms, diagnostic information, etc) transmit over from one CPS entity to another.  
\end{itemize}

An abstraction of a typical CPS architecture is shown in 
Figure~\ref{fig:cps_model}. In Figure~\ref{fig:cps_model}, $x$ denotes the physical state of the plant, $y$ captures the sensor measurements and $u$ denotes the control command computed by the PLC at any given point of time.  

\begin{figure}[t]
 \centering
 %\includegraphics[scale=0.38]{images/CPS.pdf}
 \includegraphics[scale=0.42]{cps_model3}
 \caption{An abstraction of a CPS model}
 \label{fig:cps_model}
\end{figure}

\begin{comment}
\begin{figure}[]	
	\centering
		\includegraphics[scale=0.4]{images/cps_arch} 
	%\vspace{-0.6cm}
	\caption{General architecture of CPS}
	\label{fig:cps_arch}
\end{figure}
\end{comment}





==> 11_acknowledgments.tex <==
\section*{Acknowledgment}
This work was supported by the National Research Foundation (NRF), Prime Minister's Office, Singapore, under its National Cybersecurity R\&D Programme (Award No. NRF2014NCR-NCR001-31) and administered by the National Cybersecurity R\&D Directorate.


